LongE2V: Long-Horizon Event-based Video Reconstruction, Prediction, and Frame Interpolation with Video Diffusion Models

Recovering high-quality video from sparse event streams is a challenging task. Regression methods often blur textures, while existing generative models struggle with long-term stability. We propose LongE2V, a novel approach that leverages pre-trained video diffusion priors to jointly handle event-based video reconstruction, prediction, and frame interpolation. By fine-tuning a foundational video model, our approach achieves high data efficiency and superior perceptual quality. We introduce Autoregressive Unrolling and Adaptive Context Switching to mitigate temporal drift in extremely long sequences. We also propose Reencoding Alignment with Cross Residual Correction to ensure precise bidirectional consistency during frame interpolation. Furthermore, Event Voxel Density Augmentation ensures robustness across varying sensor resolutions. Extensive experiments on real-world benchmarks demonstrate that LongE2V outperforms state-of-the-art methods across all three tasks, exhibiting exceptional temporal coherence and zero-shot generalization. Project page: https://cdfan0627.github.io/LongE2V-page/

==> 00_abstract.tex <==


\begin{abstract}
Depth-of-field control is essential in photography, but getting the perfect focus often takes several tries or special equipment. Single-image refocusing is still difficult. It involves recovering sharp content and creating realistic bokeh. Current methods have significant drawbacks. They need all-in-focus inputs, depend on synthetic data from simulators, and have limited control over aperture. We introduce \textbf{Generative Refocusing}, a two-step process that uses \emph{DeblurNet} to recover all-in-focus images from various inputs and \emph{BokehNet} for creating controllable bokeh. Our main innovation is semi-supervised training. This method combines synthetic paired data with unpaired real bokeh images, using EXIF metadata to capture real optical characteristics beyond what simulators can provide. Our experiments show we achieve top performance in defocus deblurring, bokeh synthesis, and refocusing benchmarks. Additionally, our Generative Refocusing allows text-guided adjustments and custom aperture shapes.
Project page: \texttt{\href{https://generative-refocusing.github.io/}{https://generative-refocusing.github.io/}}
% We introduce \emph{Generative Refocusing}, a single-image refocusing framework that turns any photograph—whether sharp, defocused, or mixed—into a controllable virtual camera. Our approach decomposes refocusing into two diffusion-based stages. \emph{DeblurNet} restores an all-in-focus view from a blurry input. \emph{BokehNet} then synthesizes shallow depth-of-field conditioned on a user-specified focus plane, bokeh intensity, and, optionally, aperture shape. This design removes the need for all-in-focus inputs or ground-truth depth, learns realistic optics beyond simulator bias, and supports flexible control. Central to our method is a semi-supervised training strategy: we first pre-train on synthetic pairs rendered from real all-in-focus images to enforce geometric consistency, then fine-tune on large-scale unpaired real-bokeh photographs by estimating bokeh strength and focus from EXIF metadata and depth estimates, thereby producing defocus maps that better reflect real lens behavior. Across defocus deblurring, bokeh synthesis, and refocusing, \emph{Generative Refocusing} achieves state-of-the-art results on standard benchmarks (\textsc{DPDD}, \textsc{RealDOF}) and new light-field-based datasets (\textsc{LF-Bokeh}, \textsc{LF-Refocus}).
\end{abstract}




==> 03_method.tex <==


\section{Method}
\label{sec:method}
% \noindent\textbf{Motivation and framework.}
Single-image refocusing couples two operations: recovering sharp content in out-of-focus regions and applying controllable bokeh to originally sharp areas.
Blur magnitude is dictated by a \emph{defocus map} parameterized by a user-specified \emph{focus point} and the scene \emph{depth}.
When the input is blurry, monocular depth estimation is brittle, undermining precise control over the defocus map and often yielding misfocus or artifacts.
We propose \emph{Generative Refocusing}, which decomposes the task into \emph{defocus deblurring} and \emph{bokeh synthesis}, and comprises two models, DeblurNet and BokehNet, that jointly enable precise and controllable refocusing (see Fig.~\ref{fig:pipeline} for an overview of the pipeline); 
Such a flexible pipeline allows us to exert greater control over input conditions (see Tab.~\ref{tab:method_comparison}).



\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/motivation_figuresv2.pdf}
  \caption{
    \textbf{Training data generation.}
    Each training sample consists of the following five components:
    (i) a bokeh image,
    (ii) an all-in-focus (AIF) image,
    (iii) a depth map $D$,
    (iv) a bokeh level $K$, and
    (v) a focus plane $S_1$.
    We construct these samples via three routes:
    (a) \emph{Synthetic paired data.}
    Given real AIF images and depth maps $D$, we compute a defocus map $D_{\text{def}}$ parameterized by a specified bokeh level $K$ and focus plane $S_1$, and feed it into a bokeh renderer~\cite{BokehMe} to synthesize corresponding bokeh images.
    (b) \emph{Real unpaired data.}
    Given real bokeh images, DeblurNet recovers an AIF image.
    We then estimate depth and extract a foreground mask~\cite{Zheng2024BiRefNet} to define the focus plane $S_1$.
    The bokeh level $K$ is computed from the EXIF metadata following the formulation in~\cite{Fortes2025BokehDiffusion}.
    (c) \emph{Real paired data without EXIF.}
    For real pairs lacking EXIF, we obtain a pseudo-AIF image and $S_1$ as in (b), and follow Eq.~(2) to estimate the bokeh level $K$.
    \label{fig:data_generaton}
  }
\end{figure*}

\subsection{Stage 1: Defocus Deblurring}
\noindent\textbf{DeblurNet.}
We condition the deblurring network on a pair $(I_{\text{in}}, I_{\text{pd}})$, where $I_{\text{pd}}$ is a conservative pre-deblur generated by an \emph{off-the-shelf} defocus deblurring model.
In our implementation, we use a \emph{non-generative} defocus model ~\cite{DRBNet}, whose outputs are typically content-faithful yet over-smoothed.
Our model, guided by a learned diffusion prior, then injects high-fidelity details without sacrificing geometric correctness.

\paragraph{Artifact-robust dual conditioning.}
To prevent artifacts in $I_{\text{pd}}$ from biasing the reconstruction and to ensure that fine details are recovered from $I_{\text{in}}$, we introduce two complementary mechanisms (see Fig.~\ref{fig:pipeline}\,(a)):

\begin{itemize}
  \item \emph{Positional disentanglement.}
  We encode the two inputs with \emph{disjoint} 2D positional grids: $I_{\mathrm{in}}$ is anchored at $(0,0)$, while $I_{\mathrm{pd}}$ is shifted to start at $(0,N)$, where $N$ denotes the side length of the token grid after downsampling $I_{\mathrm{in}}$.
  This shift lets the network distinguish the two sources, using $I_{\mathrm{pd}}$ as a low-frequency anchor while extracting high-frequency evidence from $I_{\mathrm{in}}$.

  \item \emph{Pre-deblur dropout.}
  During training, we stochastically replace $I_{\mathrm{pd}}$ with a zero tensor (at a fixed probability), forcing the network to remain effective when the auxiliary input is unreliable or absent.
  This regularizes the fusion, shields against method-specific artifacts, and enables the model to operate in a single-input deblurring mode at test time.
\end{itemize}





\subsection{Stage 2: Shallow Depth-of-Field Synthesis} 
\label{sec:bokehnet}

\noindent\textbf{Synthetic-pair learning.}
\emph{BokehNet} expects an AIF image, a target bokeh image, and the corresponding defocus map (see Fig.~\ref{fig:pipeline}\,(b)).
In practice, perfectly paired data and accurate defocus maps are hard to acquire.
We therefore pretrain with \emph{synthetic} pairs: starting from real all-in-focus images and their estimated depth, we randomly sample a focus plane $S_1$ and a target bokeh level $K$, and use a simulator~\cite{BokehMe} to render bokeh consistent with the induced defocus map (see Fig.~\ref{fig:data_generaton}\,(a)).
This stage quickly trains the network to modulate the circle of confusion based on the defocus map, but it remains constrained by renderer bias and may introduce non-realistic artifacts.

\medskip\noindent\textbf{Real unpaired bokeh learning.}
To capture real optics, we further leverage unpaired real bokeh images with EXIF metadata (see Fig.~\ref{fig:data_generaton}\,(b)) and estimate an \emph{approximate} bokeh level $\!K$ following \cite{Fortes2025BokehDiffusion}:
\begin{equation}
\label{eq:approxK}
K \;\approx\; \frac{f^{2}\,S_{1}}{\,2\,F\,(S_{1}-f)\,}\times \textit{pixel\_ratio},
\end{equation}
where $f$ is the focal length and $F$ denotes the \emph{aperture $f$-number}; and \textit{pixel\_ratio} compensates for sensor size and image resolution differences.
The AIF input is provided by \textbf{DeblurNet}.
Although $S_{1}$ can sometimes be read from metadata, both estimated and true depths may deviate in real scenes.
To obtain more reliable supervision, we estimate in-focus masks using BiRefNet \cite{Zheng2024BiRefNet}, and have human experts filter erroneous cases and complete partial masks.
These masks refine the focus plane and yield a consistent defocus map, enabling BokehNet to learn from real bokeh images.


\paragraph{Real paired bokeh images without metadata.}
Previous bokeh-synthesis datasets \cite{Bokehlicious} \cite{ebb} provide real pairs but omit EXIF metadata or provide insufficient fields to estimate a reliable $K$ (see Fig.~\ref{fig:data_generaton}\,(c)).
We therefore adopt a \emph{simulator-in-the-loop calibration} of the bokeh level: given an AIF image $I_{\mathrm{aif}}$, an estimated depth $D$, and a focus annotation obtained as in the unpaired setting (BiRefNet-based in-focus masks with expert filtering), we sweep $K$ and choose the value whose rendered result best matches the real bokeh target $I_{\mathrm{real}}$:
\begin{equation}
K^{\star} = \operatorname*{argmax}_{\substack{K \in \\ (K_{\min},\, K_{\max})}}
\operatorname{SSIM}\!\big(B(I_{\mathrm{aif}}, D;\, S_{1}, K),\, I_{\mathrm{real}}\big),
\end{equation}
where \emph{B} denotes our physically guided renderer and $S_{1}$ is the focus-plane proxy.
The selected $K^{\star}$ is then used as the pseudo bokeh level label for training .
Focus-plane annotation follows the same protocol as in the unpaired case.


\paragraph{Discussion.}
Although the resulting defocus maps and the AIF proxy are not perfectly accurate, this supervision regime mirrors the practical refocusing scenario.
Aggregating numbers of real bokeh images substantially improves realism and robustness over synthetic-only training.




\subsection{Bokeh-Shape Aware Synthesis}
\label{sec:shapeaware}
% \noindent\textbf{Motivation and gap.}
State-of-the-art learning-based bokeh synthesis methods deliver compelling results but \emph{do not expose} aperture-shape control.
Physics-based renderers, in principle, support arbitrary shapes, yet public implementations typically omit this functionality.
We therefore explore explicit \emph{shape-aware} control using only a bokeh shape image within a trainable framework.


% ===== RealDOF + DPDD (merged) =====
\begin{table*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.1}
  \caption{
  \textbf{Defocus deblurring benchmark on \textsc{RealDOF}~\cite{IFANet} and \textsc{DPDD}~\cite{DPDD} datasets.} We evaluate the task of recovering all-in-focus images from defocused-blur inputs. Our method, GenRefocus, uses the DeblurNet module for this task. We report both reference-based metrics (LPIPS, FID) and no-reference perceptual quality metrics (CLIP-IQA, MANIQA, MUSIQ). \colorbox{red!25}{Best}, \colorbox{orange!25}{second best}, and \colorbox{yellow!25}{third best} results are highlighted. GenRefocus outperforms all competing approaches across both benchmarks and all metrics, demonstrating the effectiveness of our diffusion-based deblurring with pre-deblur conditioning.
%   \textbf{Defocus deblurring benchmark on RealDOF~\cite{IFANet} and DPDD~\cite{DPDD}}
% \,(input: defocused-blur image $\to$ output: all-in-focus image).
% Our method GenRefocus uses the \emph{DeblurNet} module for the AIF stage.
% We highlight \colorbox{red!25}{\strut Best}, \colorbox{orange!25}{\strut Second best}, and \colorbox{yellow!25}{\strut Third best} for each metric.
% GenRefocus outperforms all competing approaches across all metrics.
}
  \label{tab:realdof_dpdd_fullwidth}
\resizebox{\textwidth}{!}{
  % \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l r r r r r r r r r r @{}}
  \begin{tabular}{lcccccccccc}
    \toprule
    & \multicolumn{5}{c}{{\textsc{RealDOF}~\cite{IFANet}}} & \multicolumn{5}{c}{{\textsc{DPDD}~\cite{DPDD}}} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11}
    {Method} &
    LPIPS $\downarrow$ & FID $\downarrow$ & CLIP\text{-}IQA $\uparrow$ & MANIQA $\uparrow$ & MUSIQ $\uparrow$ &
    LPIPS $\downarrow$ & FID $\downarrow$ & CLIP\text{-}IQA $\uparrow$ & MANIQA $\uparrow$ & MUSIQ $\uparrow$ \\
    \midrule
    Input                    & 0.5241 & 92.93 & 0.3562 & 0.2213 & 28.7087 & 0.3485 & 88.85 & 0.4337 & 0.3325 & 45.5376 \\
    GT                       & --    & --    & 0.4233 & 0.2675 & 42.5777 & --    & --    & 0.4563 & 0.3294 & 47.8102 \\
    \midrule
    AIFNet~\cite{AIFNet}     & 0.4132 & 72.38 & 0.3814 & 0.2536 & 35.7121 & 0.3090 & 79.84 & \cellcolor{yellow!25}0.4359 & \cellcolor{orange!25}0.3371 & 46.9558 \\
    IFANet~\cite{IFANet}     & 0.2994 & 33.21 & \cellcolor{orange!25}0.4088 & \cellcolor{yellow!25}0.2609 & \cellcolor{yellow!25}39.5949 & 0.2301 & 42.60 & \cellcolor{orange!25}0.4472 & 0.3276 & \cellcolor{yellow!25}47.2784 \\
    DRBNet~\cite{DRBNet}     & \cellcolor{orange!25}0.2550 & \cellcolor{yellow!25}29.89 & 0.3889 & \cellcolor{yellow!25}0.2609 & 38.9014 & \cellcolor{yellow!25}0.1819 & 39.37 & 0.4142 & 0.3254 & 46.7229 \\
    Restormer~\cite{Restormer} & 0.2863 & \cellcolor{orange!25}29.80 & \cellcolor{yellow!25}0.4062 & \cellcolor{orange!25}0.2642 & \cellcolor{orange!25}40.8355 & \cellcolor{orange!25}0.1762 & \cellcolor{orange!25}33.45 & 0.4332 & \cellcolor{yellow!25}0.3307 & \cellcolor{orange!25}47.9872 \\
    INIKNet~\cite{INIKNet}   & \cellcolor{yellow!25}0.2851 & 32.18 & 0.3984 & 0.2580 & 38.9959 & 0.1860 & \cellcolor{yellow!25}36.63 & 0.4290 & 0.3265 & 47.1961 \\
    GenRefocus (Ours)& \cellcolor{red!25}0.2356 & \cellcolor{red!25}24.73 & \cellcolor{red!25}0.4575 & \cellcolor{red!25}0.2886 & \cellcolor{red!25}43.7042 &
                                 \cellcolor{red!25}0.1598 & \cellcolor{red!25}33.08 & \cellcolor{red!25}0.4619 & \cellcolor{red!25}0.3411 & \cellcolor{red!25}49.3019 \\
    \bottomrule
  \end{tabular}
  % \end{tabular*}
  }
\end{table*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figures/visualization_of_defocus_deblur_2.pdf}
\caption{
\textbf{Qualitative comparison on defocus deblurring.} Visual results on \textbf{(a)} \textsc{RealDOF}~\cite{IFANet} and \textbf{(b)} \textsc{DPDD}~\cite{DPDD} datasets. \textcolor{blue}{Blue} boxes on the left indicate cropped regions shown in detail. Our DeblurNet faithfully recovers fine text details (``NEW YORK'') in (a) where competing methods produce blurry or distorted results. In the challenging example (b) with severe defocus blur, other methods either fail to recover structure (AIFNet~\cite{AIFNet}, DRBNet~\cite{DRBNet}, INIKNet~\cite{INIKNet}) or introduce artifacts in the background (IFANet~\cite{IFANet}, Restormer~\cite{Restormer}), while our method reconstructs geometrically consistent, visually compelling content by leveraging diffusion priors guided by the pre-deblurred input.
% \textbf{Visual comparison of defocus deblurring benchmark on (a) RealDOF \cite{IFANet} and (b) DPDD \cite{DPDD} datasets.}
}
\label{fig:defocus deblur}
\end{figure*}


\paragraph{Simulator and Data.}
Real photographs exhibiting diverse bokeh shapes are rare, and paired AIF--bokeh examples are even scarcer.
We thus rely on simulation.
A key observation is that when an all-in-focus (AIF) image lacks point-light stimuli, the simulated bokeh carries weak shape cues, making the model reluctant to learn shape-conditioned responses.
To address this, we synthesize a \emph{PointLight-1K} AIF set designed to reveal aperture shape.
We also extend the classical BokehMe renderer to \emph{scatter through a given shape}:
given an AIF image $I_{\mathrm{aif}}$, depth $D$, focus-plane proxy $S_{1}$, bokeh level $K$, and a shape kernel $s$ (binary/raster PSF), the simulator renders
\begin{equation}
\label{eq:shape-sim}
I_{\mathrm{syn}} \;=\; \mathcal{R}\!\big(I_{\mathrm{aif}}, D;\, S_{1}, K, s\big),
\end{equation}
yielding paired supervision for shape-aware training.

\paragraph{Shape-conditioned fine-tuning.}
Starting from our base model trained without shape control, we \emph{freeze all original LoRA weights} and introduce another conditioning branch that ingests a shape exemplar $s$.
Only this branch is fine-tuned while the backbone remains fixed, ensuring that \emph{shape edits do not regress} the learned bokeh synthesis.

==> 04_experiments.tex <==
\section{Experiments}

\subsection{Setup}
\label{sec:setup}

\paragraph{Backbone and training details.}
Our base generative backbone is \textsc{FLUX-1-dev} \cite{ShakkerLabs2024FluxControlNetUnionPro}, fine-tuned via LoRA \cite{hu2022lora} with a multi-condition scheme following \cite{Tan2025OminiControl2}.
\emph{DeblurNet} employs LoRA rank $r{=}128$, while \emph{BokehNet} uses $r{=}64$.

Both models are trained with per-GPU batch size $1$ and gradient accumulation over $8$ steps on $4{\times}$RTX~A6000 GPUs.
\emph{DeblurNet} is trained for $60\mathrm{K}$ steps.
\emph{BokehNet} is trained in two stages: synthetic pair training for $40\mathrm{K}$ steps and  Real unpair for another $40\mathrm{K}$ steps.


\begin{figure*}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.0}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccc}
% \includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_2284__IMG_2284_ap1_04_INPUT_zoom.jpg} & 
% \includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_2284__IMG_2284_ap1_04_GT_zoom.jpg} & 
% \includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_2284__IMG_2284_ap1_04_BokehMe_zoom.jpg} & 
% \includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_2284__IMG_2284_ap1_04_Bokehlicious_zoom.jpg} & 
% \includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_2284__IMG_2284_ap1_04_BokehDiff_zoom.jpg} & 
% \includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_2284__IMG_2284_ap1_04_Ours_zoom.jpg} \\
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_5683__IMG_5683_ap1_02_INPUT_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_5683__IMG_5683_ap1_02_GT_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_5683__IMG_5683_ap1_02_BokehMe_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_5683__IMG_5683_ap1_02_Bokehlicious_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_5683__IMG_5683_ap1_02_BokehDiff_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_5683__IMG_5683_ap1_02_Ours_zoom.jpg} \\
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_3778__IMG_3778_ap2_00_INPUT_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_3778__IMG_3778_ap2_00_GT_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_3778__IMG_3778_ap2_00_BokehMe_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_3778__IMG_3778_ap2_00_Bokehlicious_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_3778__IMG_3778_ap2_00_BokehDiff_zoom.jpg} & 
\includegraphics[width=0.17\textwidth]{figures/bokeh_visual/IMG_3778__IMG_3778_ap2_00_Ours_zoom.jpg} \\
Input & GT & BokehMe~\cite{BokehMe} & Bokehlicious~\cite{Bokehlicious} & BokehDiff~\cite{BokehDiff} & Ours \\
\end{tabular}
}
\caption{
\textbf{Qualitative comparison on bokeh synthesis benchmark.} Results on \textsc{LF-Bokeh} with zoomed patches (\textcolor{blue}{blue} and \textcolor{orange}{orange} boxes) highlighting detail quality. Our BokehNet synthesizes bokeh effects that better match ground truth with realistic blur gradients and natural occlusion handling. Baselines show various artifacts: BokehMe~\cite{BokehMe} exhibits simulator bias, Bokehlicious~\cite{Bokehlicious} over-smooths details, and BokehDiff~\cite{BokehDiff} produces inconsistent defocus. Our semi-supervised training on real bokeh images enables the capture of authentic lens characteristics.
% \textbf{visual comparison of bokeh benchmark our \textsc{LF-Bokeh}.}
}
\label{fig:refocus}
\end{figure*}

\paragraph{Datasets.}
We summarize the training data for the two modules below.

\noindent\textit{DeblurNet.} We train on \textsc{DPDD}~\cite{DPDD} together with a curated subset of \textsc{RealBokeh\_3MP}~\cite{Bokehlicious}, totaling approximately 4.5K image pairs.

\noindent\textit{BokehNet (synthetic pairs).} We use AIF images from~\cite{yuan2025generative} and a subset of \emph{EBB!}~\cite{ebb}, and procedurally render defocus under varying aperture sizes/shapes and focus points to generate about 70K synthetic pairs.

\textit{BokehNet (real supervision).} We incorporate (i) an unpaired real-bokeh set collected from Flickr by Fortes et al.~\cite{Fortes2025BokehDiffusion}, and (ii) real AIF–bokeh pairs with incomplete metadata from \textsc{RealBokeh\_3MP}~\cite{Bokehlicious} and \textsc{LFDOF}~\cite{AIFNet}, contributing approximately 27K real examples in total.
% 
% \noindent All datasets are used strictly for research, and we ensure no scene overlaps between training and evaluation splits.
% 
All datasets are used strictly for research and are split so that no scene overlaps across training and evaluation.


\begin{table}[t]
\centering
\small
\caption{
\textbf{Bokeh synthesis benchmark.} 
Evaluation on \textsc{LF-Bokeh} (200 light-field images with multiple focus planes). 
Following~\cite{BokehDiff}, we use per-image binary search for optimal $K$. 
$^\dagger$Bokehlicious supports only aperture size control. 
Our semi-supervised training on real bokeh data outperforms all baselines.
% \textbf{Quantitative comparisons on our bokeh synthesis benchmark \textsc{LF-Bokeh}.} Our method \textbf{GenRefocus (Ours)} uses the \emph{BokehNet} module for the AIF stage. We compare against current SOTA bokeh models and outperform them across all metrics. \quad {\footnotesize\textsuperscript{†}Bokehlicious can only adjust the aperture size.}
}
\label{tab:bokeh}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
Method & LPIPS~$\downarrow$ & DISTS~$\downarrow$ & CLIP-I~$\uparrow$ \\
\midrule
BokehMe \cite{BokehMe}                  & \cellcolor{orange!25}0.1228 & \cellcolor{orange!25}0.0744 & \cellcolor{orange!25}0.9511 \\
Bokehlicious$^{\dagger}$ \cite{Bokehlicious} & 0.1799 & 0.1062 & \cellcolor{yellow!25}0.9304 \\
BokehDiff \cite{BokehDiff}                & \cellcolor{yellow!25}0.1708 & \cellcolor{yellow!25}0.0933 & 0.9192 \\
GenRefocus (Ours) & \cellcolor{red!25}0.1047 & \cellcolor{red!25}0.0611 & \cellcolor{red!25}0.9570 \\
\bottomrule
\end{tabular}
% }
\end{table}



\paragraph{Benchmarks.}
We evaluate three tasks: (i) \emph{defocus deblurring} on \textsc{DPDD} and \textsc{RealDOF};
(ii) \emph{bokeh synthesis} on our new \textsc{LF-Bokeh} benchmark, comprising $200$ images with multiple focus planes synthesized from \cite{EPFL} and \cite{Dansereau2019LIFF} light-field captures;
and (iii) \emph{refocusing} on \textsc{LF-Refocus}, built by pairing same-scene images within \textsc{LF-Bokeh} to form $400$ source--target pairs.

\paragraph{Inference-time resolution and aspect ratio.}
We adopt a tiling strategy inspired by ~\cite{multidiffusion} at evaluation time: we split the input image into overlapping patches and perform tile-wise denoising before blending them back together. As a result, all benchmarks are conducted at each dataset's original aspect ratio and resolution, without additional resizing.

\subsection{Comparison}
\label{sec:comparison}




\paragraph{Defocus deblurring.}
As stated on Tab.~\ref{tab:realdof_dpdd_fullwidth},  \emph{DeblurNet} consistently outperforms all baselines across reference and no-reference metrics. On certain NR-IQA measures, it even surpasses the ground-truth. 
% 
Qualitatively, Fig.~\ref{fig:defocus deblur} (a) shows faithful recovery of the “NEW YORK” text with well-preserved edges. 
The scene in Fig.~\ref{fig:defocus deblur} (b) is particularly challenging: competing methods recover only a blurry dark stripe and further distort the background, whereas \emph{DeblurNet} reconstructs structure-consistent content and delivers visually compelling results without introducing artifacts or geometry drift.




% ===== refocus =====

\begin{table*}[t]
  \centering
  \small
  % \setlength{\tabcolsep}{5pt}
  % \renewcommand{\arraystretch}{1.1}
  \caption{
  \textbf{Quantitative comparison on refocusing benchmark.} Results on our \textsc{LF-Refocus} dataset (400 pairs with different focus planes). We compare our DeblurNet+BokehNet pipeline against combinations of existing all-in-focus estimation methods~\cite{DRBNet,Restormer} and bokeh synthesis methods~\cite{BokehMe,BokehDiff}. Optimal bokeh level $K$ is determined via per-image binary search following~\cite{BokehDiff}. 
  % \colorbox{red!25}{Best}, \colorbox{orange!25}{second}, \colorbox{yellow!25}{third} best shown. 
  Our approach achieves superior performance across all metrics, demonstrating the benefit of joint optimization and semi-supervised training.
%   \textbf{Quantitative comparisons on our refocusing benchmark \textsc{LF-Refocus}.}
% For refocusing, since no existing method performs the task end-to-end, we build strong baselines by combining (1) all-in-focus (AiF) estimation~\cite{DRBNet,Restormer} with (2) bokeh synthesis~\cite{BokehMe,BokehDiff}. Our proposed \textbf{GenRefocus} performs favorably against these strong baselines across perceptual and no-reference metrics.
}
  \label{tab:refocus}
  \begin{tabular}{llcccccc}
    \toprule
    {AiF Estimation} & {Bokeh Synthesis} & {LPIPS} $\downarrow$ & {DISTS} $\downarrow$ & {CLIP-I} $\uparrow$ & {MUSIQ} $\uparrow$ & {NIQE} $\downarrow$ & {CLIP-IQA} $\uparrow$ \\
    \midrule
    \multirow{2}{*}{DRBNet \cite{DRBNet}}        & BokehMe \cite{BokehMe}   & \cellcolor{orange!25}0.1471 & \cellcolor{orange!25}0.0937 & \cellcolor{orange!25}0.9335 & 43.3087 & 6.5783 & 0.4460 \\
                                                 & BokehDiff \cite{BokehDiff} & 0.1848 & 0.1030 & 0.9310 & \cellcolor{orange!25}48.0766 & \cellcolor{orange!25}5.8195 & \cellcolor{yellow!25}0.4997 \\
    \multirow{2}{*}{Restormer \cite{Restormer}} & BokehMe \cite{BokehMe}   & \cellcolor{yellow!25}0.1554 & \cellcolor{yellow!25}0.0963 & 0.9303 & 43.3188 & 7.1249 & 0.4782 \\
                                                 & BokehDiff \cite{BokehDiff} & 0.1860 & 0.1016 & \cellcolor{yellow!25}0.9320 & \cellcolor{yellow!25}48.0326 & \cellcolor{yellow!25}6.3216 & \cellcolor{orange!25}0.5352 \\
    DeblurNet (Ours)                             & BokehNet (Ours)          & \cellcolor{red!25}0.1458 & \cellcolor{red!25}0.0850 & \cellcolor{red!25}0.9451 & \cellcolor{red!25}52.6954 & \cellcolor{red!25}5.3343 & \cellcolor{red!25}0.5763 \\
    \bottomrule
  \end{tabular}
\end{table*}




\paragraph{Bokeh synthesis.}
Following the BokehDiff protocol~\cite{BokehDiff}, we conduct a per-image \emph{binary search} over the bokeh level $K$ and select the value that \emph{maximizes SSIM} with the target.
All other control signals are held fixed, ensuring a fair comparison in which each method operates at its best attainable setting.
As summarized in Tab.~\ref{tab:bokeh}, our approach attains the highest scores on both fidelity and perceptual metrics, outperforming all baselines.
% 
The qualitative results in Fig.~\ref{fig:refocus} show that our method synthesizes bokeh that more closely matches that of real photographs. In the zoomed-in patches, our outputs more faithfully reproduce the ground-truth bokeh than competing baselines. Other methods tend to naively translate the predicted defocus map into blur strength, so any error in the depth scale directly leads to over- or under-blurring. In contrast, \emph{BokehNet}, trained with our semi-supervised strategy, is more robust to such depth-scale inaccuracies and thus produces a more appropriate amount of blur that better matches the ground truth.


\paragraph{Refocusing.}
We build \emph{four} two-stage baselines by pairing strong AIF estimators (DRBNet~\cite{DRBNet}, Restormer~\cite{Restormer}) with bokeh synthesizers (BokehMe~\cite{BokehMe}, BokehDiff~\cite{BokehDiff}), yielding the $2\times2$ combinations.
For each method, we also follow the protocol of BokehDiff~\cite{BokehDiff} to select the best bokeh level $K$ .
% 
As shown in Tab.\ref{tab:refocus}, our approach achieves the best results on both fidelity and perceptual metrics, outperforming all baseline pairings.
% 
Qualitatively, Fig.~\ref{fig:refocus_depth_visual} shows that competing methods tend to produce spatially ambiguous blur and fail to place the focal plane correctly, resulting in uniformly soft content and inaccurate foreground/background separation.
In contrast, our approach restores fine details at the intended focus while synthesizing physically consistent bokeh elsewhere.

\begin{figure*}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.0}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccc}
\includegraphics[width=0.14\textwidth]{figures/visual/10/IMG_5359_ap1_00_input_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/10/IMG_5359__IMG_5359_ap1_00.png__IMG_5359_ap1_04_GT_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/10/IMG_5359__IMG_5359_ap1_00.png__IMG_5359_ap1_04_DRBNetXbokehme_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/10/IMG_5359__IMG_5359_ap1_00.png__IMG_5359_ap1_04_DRBNetXbokehdiff_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/10/IMG_5359__IMG_5359_ap1_00.png__IMG_5359_ap1_04_RestformerXbokehme_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/10/IMG_5359__IMG_5359_ap1_00.png__IMG_5359_ap1_04_RestformerXbokehdiff_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/10/IMG_5359__IMG_5359_ap1_00.png__IMG_5359_ap1_04_ours_zoom.jpg} \\
% \includegraphics[width=0.14\textwidth]{figures/visual/15/IMG_4173_ap1_00_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/15/IMG_4173__IMG_4173_ap1_00.png__IMG_4173_ap1_04_GT_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/15/IMG_4173__IMG_4173_ap1_00.png__IMG_4173_ap1_04_DRBNetXbokehme_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/15/IMG_4173__IMG_4173_ap1_00.png__IMG_4173_ap1_04_DRBNetXbokehdiff_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/15/IMG_4173__IMG_4173_ap1_00.png__IMG_4173_ap1_04_RestformerXbokehme_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/15/IMG_4173__IMG_4173_ap1_00.png__IMG_4173_ap1_04_RestformerXbokehdiff_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/15/IMG_4173__IMG_4173_ap1_00.png__IMG_4173_ap1_04_ours_zoom.jpg} \\
\includegraphics[width=0.14\textwidth]{figures/visual/25/IMG_6245_ap2_01_input_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/25/IMG_6245__IMG_6245_ap2_01.png__IMG_6245_ap1_04_GT_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/25/IMG_6245__IMG_6245_ap2_01.png__IMG_6245_ap1_04_DRBNetXbokehme_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/25/IMG_6245__IMG_6245_ap2_01.png__IMG_6245_ap1_04_DRBNetXbokehdiff_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/25/IMG_6245__IMG_6245_ap2_01.png__IMG_6245_ap1_04_RestformerXbokehme_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/25/IMG_6245__IMG_6245_ap2_01.png__IMG_6245_ap1_04_RestformerXbokehdiff_zoom.jpg} & \includegraphics[width=0.14\textwidth]{figures/visual/25/IMG_6245__IMG_6245_ap2_01.png__IMG_6245_ap1_04_ours_zoom.jpg} \\
Input & GT & DRBNet~\cite{DRBNet} & DRBNet~\cite{DRBNet} & Restormer~\cite{Restormer} & Restormer~\cite{Restormer} & GenRefocus \\
 & &  + BokehMe~\cite{BokehMe} &  + BokehDiff~\cite{BokehDiff} &  + BokehMe~\cite{BokehMe} &  + BokehDiff~\cite{BokehDiff} &  (Ours) \\
\end{tabular}
}
% \includegraphics[height=\textheight,keepaspectratio]{figures/visualization_of_refocusing.pdf}
\caption{
\textbf{Qualitative comparison on refocusing benchmark.} Results on \textsc{LF-Refocus} comparing our end-to-end trained pipeline against baseline combinations of existing deblurring~\cite{DRBNet,Restormer} and bokeh synthesis~\cite{BokehMe,BokehDiff} methods. Zoomed patches (\textcolor{blue}{blue} and \textcolor{orange}{orange} boxes) highlight focal and defocused regions. Baselines struggle with accurate focus-plane placement and produce inconsistent or overly smooth blur. Our method achieves sharp refocusing at the target plane while synthesizing photorealistic bokeh, closely matching ground truth across diverse scenes.
% \textbf{Visual comparison on our \textsc{LF-Refocus}.} Our method refocuses the target regions, yielding crisper details and cleaner boundaries while maintaining realistic defocus elsewhere, consistently outperforming prior baselines.
}
\label{fig:refocus_depth_visual}
\end{figure*}


% ===== ablation of one step two stage =====
\begin{table}[t]
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.1}
  \caption{
\textbf{Ablation on pipeline design.} 
Comparing one-stage (direct refocusing) and two-stage (deblur then re-bokeh) on \textsc{LF-Refocus}. 
Both use the same backbone and synthetic data. 
Two-stage enables better depth control and independent semi-supervised learning per stage, yielding substantial improvements.
  % \textbf{Ablation of one stage and two stage refocusing}. we evaluate the one stage refocus on refocusing task comparing with our two stage method.
  }
  \label{tab:ablation-refocus} % 避免 label 內有空白
  \begin{tabular}{lccc}
    \toprule
    Method  & LPIPS~$\downarrow$ & DISTS~$\downarrow$ & CLIP-I~$\uparrow$\\
    \midrule
    One stage         & 0.1723 & 0.0976 & 0.9345  \\
    \rowcolor{black!10}
    Two stage (ours) & \textbf{0.1458} & \textbf{0.0850} & \textbf{0.9461} \\
    \bottomrule
  \end{tabular}
\end{table}

% ===== Ablation: training regime (synthetic-only vs semi-supervised fine-tune) =====
\begin{table}[t]
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.1}
  \caption{
  \textbf{Ablation on BokehNet training.} 
Comparing synthetic-only vs. adding real unpaired bokeh images on \textsc{LF-Bokeh}. 
Second stage uses real bokeh with estimated parameters (\cref{sec:bokehnet}), initialized from synthetic weights. 
Real data enables learning authentic optical characteristics beyond simulators.
  % \textbf{Ablation on BokehNet training strategy.} We compare (i) \emph{Synthetic pair} training and (ii) \emph{Synthetic pair+ Real unpair} fine-tuning initialized from the \emph{Synthetic pair} weight.
  }
  \label{tab:ablation-train}
  \begin{tabular}{lccc}
    \toprule
    Method & LPIPS~$\downarrow$ & DISTS~$\downarrow$ & CLIP-I~$\uparrow$ \\
    \midrule
    Synthetic pair   & 0.1289 & 0.0738 & 0.9461  \\
    \rowcolor{black!10}
    Synthetic pair+ Real unpair  & \textbf{0.1047} & \textbf{0.0611} & \textbf{0.9570}  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Ablation Study}
\paragraph{One stage and two stage refocusing.}
We also evaluate a variant that takes an input image and a provided defocus map and \emph{directly} produces a refocused output in a single pass.
Concretely, we instantiate a one-stage model by reusing the \emph{BokehNet} backbone and training it on the same synthetic pairs, then assess it on the refocusing benchmark.
As reported in Tab.~\ref{tab:ablation-refocus}, the one-stage variant lags the proposed two-stage pipeline by a substantial margin.
% 
We attribute this gap to two factors.
First, \emph{control fidelity}: the defocus map relies on depth estimated from a \emph{blurry} input; without an all-in-focus view, depth quality degrades, leading to misaligned or biased blur fields and weakening refocusing accuracy.
Second, \emph{data leverage}: the one-stage formulation cannot separate the problem into defocus removal and bokeh synthesis, preventing us from injecting real-data supervision tailored to each subtask.

\paragraph{Key idea and BokehNet training ablation.}
Our core idea is to use \emph{data generation} to harvest real-world supervision for training BokehNet, leveraging \emph{real unpaired} images.
% 
To quantify its impact, we evaluate two training settings without introducing additional architectural changes:
(i) \emph{synthetic pair}: BokehNet is trained purely on synthetic paired data; and
(ii) \emph{synthetic pair + real unpaired}: starting from (i), we further train with real unpaired images processed by our pipeline to produce usable supervision.
% 
On the bokeh-synthesis benchmark, the \emph{synthetic pair} setting performs on par with a classical simulator baseline, while the \emph{synthetic pair + real-unpaired} setting delivers substantial improvements across both fidelity and perceptual metrics (Tab.~\ref{tab:ablation-train}).

\paragraph{Application.} As illustrated in Fig.~\ref{fig:bokeh shape}, after we fine-tune BokehNet on our point-light 1K dataset, the model can synthesize bokeh with diverse, user-specified aperture shapes.
Moreover, even though DeblurNet is trained without any text prompts, it can still leverage textual instructions at inference time to refine the all-in-focus output, as shown in Fig.~\ref{fig:text_correction}.
This highlights a key advantage of generative defocus-deblurring models: they naturally support post-hoc, prompt-based correction and editing of the reconstructed content.























\begin{figure}[t]
\centering
\small
\setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{1.0}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccc}
\includegraphics[width=0.25\columnwidth]{figures/shape/shape_input.jpg} & 
\includegraphics[width=0.25\columnwidth]{figures/shape/shape_tri.jpg} & 
\includegraphics[width=0.25\columnwidth]{figures/shape/shape_heart.jpg} & 
\includegraphics[width=0.25\columnwidth]{figures/shape/shape_star.jpg} \\
Input & Triangle & Heart & Star \\
\end{tabular}
}
\caption{
\textbf{Controllable aperture shape synthesis.} Given an input image, our BokehNet can synthesize bokeh effects with custom aperture shapes (triangle, heart, star) by conditioning on shape exemplars. Background point lights exhibit the specified aperture geometry while maintaining scene consistency. 
% \textbf{Flexible bokeh shape control.} 
% By using the chosen aperture shape, GenRefocus produces images featuring the corresponding bokeh while maintaining high fidelity to the original image content.
}
\label{fig:bokeh shape}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/text_guidance.pdf}
\caption{
\textbf{Text-guided deblurring.} 
DeblurNet uses optional text prompts to guide reconstruction of severely blurred text. 
With prompts, we correct hallucinations (red: ``DESION'' $\rightarrow$ ``DESIGN'') and recover accurate text (green: ``yeurs'' $\rightarrow$ ``years''), matching GT. 
Without guidance, it hallucinates incorrect content.
% This capability emerges from FLUX's pre-trained text-to-image prior without requiring text conditioning during training.
% \textbf{Text-guided defocus deblurring with DeblurNet.}
% We can inject a text prompt during inference even if text does not provide during training.
% With the prompt \emph{``WE DESIGN LOGISTICS, DELIVERING TRUST. Beneath the golden `90' logo, the word `years SINCE 1930' in smaller font.''},
% the model corrects hallucinated characters in the deblurred output (e.g., \emph{desion}~$\rightarrow$~\emph{design}, \emph{yeurs}~$\rightarrow$~\emph{years}).
}
\label{fig:text_correction}
\end{figure}


